Regularizing Towards Soft Equivariance Under Mixed Symmetries

Datasets often have their intrinsic symmetries, and particular deep-learning models called equivariant or invariant models have been developed to exploit these symmetries. However, if some or all of these symmetries are only approximate, which frequently happens in practice, these models may be suboptimal due to the architectural restrictions imposed on them. We tackle this issue of approximate symmetries in a setup where symmetries are mixed, i.e., they are symmetries of not single but multiple different types and the degree of approximation varies across these types. Instead of proposing a new architectural restriction as in most of the previous approaches, we present a regularizer-based method for building a model for a dataset with mixed approximate symmetries. The key component of our method is what we call equivariance regularizer for a given type of symmetries, which measures how much a model is equivariant with respect to the symmetries of the type. Our method is trained with these regularizers, one per each symmetry type, and the strength of the regularizers is automatically tuned during training, leading to the discovery of the approximation levels of some candidate symmetry types without explicit supervision. Using synthetic function approximation and motion forecasting tasks, we demonstrate that our method achieves better accuracy than prior approaches while discovering the approximate symmetry levels correctly.

==> main/misc.tex <==

\section*{Accessibility}
Authors are kindly asked to make their submissions as accessible as possible for everyone including people with disabilities and sensory or neurological differences.
Tips of how to achieve this and what to pay attention to will be provided on the conference website \url{http://icml.cc/}.

\section*{Software and Data}

If a paper is accepted, we strongly encourage the publication of software and data with the
camera-ready version of the paper whenever appropriate. This can be
done by including a URL in the camera-ready copy. However, \textbf{do not}
include URLs that reveal your institution or identity in your
submission for review. Instead, provide an anonymous URL or upload
the material as ``Supplementary Material'' into the CMT reviewing
system. Note that reviewers are not required to look at this material
when writing their review.

% % Acknowledgements should only appear in the accepted version.
% \section*{Acknowledgements}

% \textbf{Do not} include acknowledgements in the initial version of
% the paper submitted for blind review.

% If a paper is accepted, the final camera-ready version can (and
% probably should) include acknowledgements. In this case, please
% place such acknowledgements in an unnumbered section at the
% end of the paper. Typically, this will include thanks to reviewers
% who gave useful comments, to colleagues who contributed to the ideas,
% and to funding agencies and corporate sponsors that provided financial
% support.


==> tables/model_parameters.tex <==
\begin{table}[ht]
    \caption{The number of parameters of baseline models and our model on each dataset.}
    \centering
    % \scriptsize
    \vskip 0.05in
    \def\arraystretch{1.1}
    \resizebox{0.6\columnwidth}{!}{
        \begin{tabular}{lccc}
            \toprule
            Method      &   PhysioNet 2012 &  MIMIC-III       & Human Activity \\
            \midrule
            GRU-Mean    &          226,817  &          210,689 &  84,647        \\
            GRU-Simple  &          351,745 &          301,569 &  85,117        \\
            GRU-Forward &          294,145 &          276,225 &  85,687        \\
            GRU-D       &          332,363 &          292,897 &  86,566        \\
            PhasedLSTM  &          511,745 &          445,441 &       -        \\
            IP-Nets     &          353,151 &          301,841 &       -        \\
            Ours        &          262,980 &          224,305 &  84,251        \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:model_parameters}
\end{table}

==> tables/oodmse_inertia.tex <==

\begin{table}[!t]
    \caption{OOD MSE results in the function-approximation tasks}
    \centering
    % \scriptsize
    \vskip 0.05in
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{lllll}
            \toprule
   Task (Symmetry group) & EMLP & RPP & Mixed RPP & MLP w/ PER\\
            \midrule
            % \multirow{1}{*}{Distance (no error)}& 0 \textpm0 & 0 \textpm0 & 0 \textpm0 & 0 \textpm0\\ 
            % \multirow{1}{*}{Distance (l2 norm error)}& 0 \textpm0 & 0 \textpm0 & 0 \textpm0 & 0 \textpm0\\ 
            % \multirow{1}{*}{Distance (l1 diff error)}& 0 \textpm0 & 0 \textpm0 & 0 \textpm0 & 0 \textpm0\\ 
            \multirow{1}{*}{Inertia ($\text{O}(3)$)} & \textbf{0.16 \textpm0.02} & 57.05 \textpm16.74 & - &  0.62 \textpm0.57 \\
            \multirow{1}{*}{Inertia ($\text{O}^x(2)$)} &  18.95\textpm10.77& 45.35 \textpm14.31 & \textbf{12.92 \textpm1.57} & 25.27 \textpm2.45 \\ 
            \multirow{1}{*}{Inertia ($\text{O}^y(2)$)} & 20.13 \textpm7.17 & 46.46 \textpm9.70 &  \textbf{11.78\textpm1.95} &  23.41 \textpm6.62 \\ 
            \multirow{1}{*}{Inertia ($\text{O}^z(2)$)} & 25.33 \textpm25.35 & 47.00 \textpm8.71 & \textbf{14.48 \textpm7.14} &  26.82 \textpm1.60 \\
            \multirow{1}{*}{Inertia (-)} & 0.09 \textpm0.02 & 36.48 \textpm12.85 & - &  \textbf{0.18 \textpm0.13} \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:ood-function}
\end{table}

==> tables/table_template.tex <==

\begin{table}[!t]
    \caption{OOD MSE results in function-approximation tasks}
    \centering
    % \scriptsize
    \vskip 0.05in
    \resizebox{0.7\columnwidth}{!}{
        \begin{tabular}{lllll}
            \toprule
   Task & EMLP & RPP & Mixed RPP & PER\\
            \midrule
            \multirow{1}{*}{Distance}& 0\textpm0 & 0\textpm0 & 0\textpm0 & 0\textpm0\\ 
            \multirow{1}{*}{Inertia (x-axis noise)} &  0\textpm0& 0\textpm0 & 0\textpm0 & 0\textpm0 \\ 
            \multirow{1}{*}{Inertia (y-axis noise)} & 0\textpm0 & 0\textpm0 &  0\textpm0 &  0\textpm0 \\ 
            \multirow{1}{*}{Inertia (z-axis noise)} & 0\textpm0 & 0\textpm0 & 0\textpm0 &  0\textpm0 \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:type1_cnn}
\end{table}

==> tables/testmse_motion.tex <==

\begin{table}[!t]
    \caption{\revise{Test ADE results in the motion forecasting task}}
    \centering
    % \scriptsize
    \vskip 0.05in
        \begin{tabular}{llllll}
            \toprule
   Models & ADE ($\times 10^{-2}$)\\
            \midrule
            \multirow{1}{*}{$\text{O}^z(2)$EMLP}& 1.66\textpm0.27\\
            \multirow{1}{*}{$\text{O}(3)$EMLP}& 0.69\textpm0.24\\
            \multirow{1}{*}{$\text{O}(3)$RPP}& 0.92\textpm0.48\\
            \multirow{1}{*}{$\text{O}(3)$RPP-$\text{O}^z(2)$EMLP}& 55.49\textpm122.32\\
            \multirow{1}{*}{MLP-\big($\text{O}^x(2),\text{O}^y(2),\text{O}^z(2)$\big)PER}& \textbf{0.42\textpm0.13}\\
            \bottomrule
        \end{tabular}
    \label{tab:test-motion}
\end{table}
